Knowledge Graph Refinement based on Triplet BERT-Networks

Knowledge graph embedding techniques are widely used for knowledge graph refinement tasks such as graph completion and triple classification. These techniques aim at embedding the entities and relations of a Knowledge Graph (KG) in a low dimensional continuous feature space. This paper adopts a transformer-based triplet network creating an embedding space that clusters the information about an entity or relation in the KG. It creates textual sequences from facts and fine-tunes a triplet network of pre-trained transformer-based language models. It adheres to an evaluation paradigm that relies on an efficient spatial semantic search technique. We show that this evaluation protocol is more adapted to a few-shot setting for the relation prediction task. Our proposed GilBERT method is evaluated on triplet classification and relation prediction tasks on multiple well-known benchmark knowledge graphs such as FB13, WN11, and FB15K. We show that GilBERT achieves better or comparable results to the state-of-the-art performance on these two refinement tasks.

==> src/pgfplots__Diagram__1.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        


\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,596); %set diagram left start at 0, and has height of 596

%Rounded Rect [id:dp49752108198300404] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (75.1,35.37) .. controls (75.1,33.92) and (76.28,32.75) .. (77.73,32.75) -- (85.59,32.75) .. controls (87.04,32.75) and (88.22,33.92) .. (88.22,35.37) -- (88.22,64.29) .. controls (88.22,65.74) and (87.04,66.91) .. (85.59,66.91) -- (77.73,66.91) .. controls (76.28,66.91) and (75.1,65.74) .. (75.1,64.29) -- cycle ;
%Rounded Rect [id:dp5275448882383111] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (75.1,77.05) .. controls (75.1,75.6) and (76.28,74.43) .. (77.73,74.43) -- (85.59,74.43) .. controls (87.04,74.43) and (88.22,75.6) .. (88.22,77.05) -- (88.22,105.97) .. controls (88.22,107.42) and (87.04,108.59) .. (85.59,108.59) -- (77.73,108.59) .. controls (76.28,108.59) and (75.1,107.42) .. (75.1,105.97) -- cycle ;
%Rounded Rect [id:dp9931086331717305] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (75.1,118.05) .. controls (75.1,116.6) and (76.28,115.42) .. (77.73,115.42) -- (85.59,115.42) .. controls (87.04,115.42) and (88.22,116.6) .. (88.22,118.05) -- (88.22,146.96) .. controls (88.22,148.41) and (87.04,149.59) .. (85.59,149.59) -- (77.73,149.59) .. controls (76.28,149.59) and (75.1,148.41) .. (75.1,146.96) -- cycle ;
%Straight Lines [id:da6877156241088023] 
\draw    (28.48,32.07) -- (39.82,44.15) ;
\draw [shift={(41.88,46.33)}, rotate = 226.8] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da725412245619319] 
\draw    (28.48,32.07) -- (41.18,85.47) ;
\draw [shift={(41.88,88.39)}, rotate = 256.62] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da1395740704639994] 
\draw    (28.48,32.07) -- (37.59,126.43) ;
\draw [shift={(37.88,129.42)}, rotate = 264.49] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da535715350494375] 
\draw    (89.67,49.15) -- (109.53,49.15) ;
\draw [shift={(111.53,49.15)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7402428496268327] 
\draw    (89.67,90.14) -- (109.53,90.14) ;
\draw [shift={(111.53,90.14)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6212801540532888] 
\draw    (89.67,130.45) -- (109.53,130.45) ;
\draw [shift={(111.53,130.45)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp3025847002765598] 
\draw   (115.9,38.22) -- (152.32,38.22) -- (152.32,56.66) -- (115.9,56.66) -- cycle ;
%Shape: Rectangle [id:dp6551608395583364] 
\draw   (115.9,79.89) -- (152.32,79.89) -- (152.32,98.34) -- (115.9,98.34) -- cycle ;
%Shape: Rectangle [id:dp6338690857153744] 
\draw   (115.9,118.84) -- (152.32,118.84) -- (152.32,137.29) -- (115.9,137.29) -- cycle ;
%Shape: Ellipse [id:dp9514920666867486] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (105.7,87.07) .. controls (105.7,51.03) and (118.58,21.82) .. (134.48,21.82) .. controls (150.37,21.82) and (163.25,51.03) .. (163.25,87.07) .. controls (163.25,123.1) and (150.37,152.32) .. (134.48,152.32) .. controls (118.58,152.32) and (105.7,123.1) .. (105.7,87.07) -- cycle ;
%Straight Lines [id:da33141923184673505] 
\draw    (153.78,47.78) -- (188.21,47.78) ;
\draw [shift={(190.21,47.78)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9629853152536678] 
\draw    (154.51,90.14) -- (189.66,90.14) ;
\draw [shift={(191.66,90.14)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da01517255683547325] 
\draw    (155.24,127.72) -- (190.39,127.72) ;
\draw [shift={(192.39,127.72)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4485086177379709] 
\draw    (218.36,126.71) -- (304,125.61) ;
\draw [shift={(306,125.59)}, rotate = 179.27] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da30490242243400734] 
\draw    (218.36,126.71) -- (216.91,40.13) ;
\draw [shift={(216.88,38.13)}, rotate = 89.04] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp711843316858245] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (271.96,39.92) .. controls (271.96,41.62) and (273.42,42.99) .. (275.24,42.99) .. controls (277.05,42.99) and (278.51,41.62) .. (278.51,39.92) .. controls (278.51,38.22) and (277.05,36.84) .. (275.24,36.84) .. controls (273.42,36.84) and (271.96,38.22) .. (271.96,39.92) -- cycle ;
%Shape: Ellipse [id:dp5087799402141548] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (274.7,106.55) .. controls (274.7,108.24) and (276.17,109.62) .. (277.98,109.62) .. controls (279.79,109.62) and (281.26,108.24) .. (281.26,106.55) .. controls (281.26,104.85) and (279.79,103.47) .. (277.98,103.47) .. controls (276.17,103.47) and (274.7,104.85) .. (274.7,106.55) -- cycle ;
%Shape: Ellipse [id:dp46712950038259216] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (233.01,70.5) .. controls (233.01,72.1) and (234.39,73.4) .. (236.1,73.4) .. controls (237.81,73.4) and (239.2,72.1) .. (239.2,70.5) .. controls (239.2,68.9) and (237.81,67.59) .. (236.1,67.59) .. controls (234.39,67.59) and (233.01,68.9) .. (233.01,70.5) -- cycle ;
%Straight Lines [id:da7204966907605135] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (209.15,48.46) -- (236.1,67.59) ;
%Straight Lines [id:da21930181596685938] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (210.97,88.43) -- (271.96,39.92) ;
%Straight Lines [id:da5922938696867524] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (209.15,126.35) -- (274.7,106.55) ;
%Straight Lines [id:da7813386207001465] 
\draw    (241.95,76.46) -- (273.23,105.19) ;
\draw [shift={(274.7,106.55)}, rotate = 222.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
\draw [shift={(240.47,75.11)}, rotate = 42.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
%Curve Lines [id:da947737416826558] 
\draw    (252,71.89) .. controls (266.23,70.8) and (275.68,58.96) .. (277.98,54.06) ;
\draw [shift={(277.98,54.06)}, rotate = 261.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(252,71.89)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (38.53,40.31) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{24.55pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize anchor}
\end{center}

\end{minipage}};
% Text Node
\draw (35.18,84.04) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{26.93pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize positive}
\end{center}

\end{minipage}};
% Text Node
\draw (31.35,125.37) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{29.72pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize negative}
\end{center}

\end{minipage}};
% Text Node
\draw (19,9.9) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{58.41pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Train triple (s,p,o)}
\end{center}

\end{minipage}};
% Text Node
\draw (123.9,40.51) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{16.61pt}\setlength\topsep{0pt}
\begin{center}
{\tiny \textbf{BERT}}
\end{center}

\end{minipage}};
% Text Node
\draw (100.89,151.94) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{50.75pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize shared weights}
\end{center}

\end{minipage}};
% Text Node
\draw (151.5,28) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.35pt}\setlength\topsep{0pt}
\begin{center}
{\tiny mean pooling}
\end{center}

\end{minipage}};
% Text Node
\draw (150.32,70.71) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.35pt}\setlength\topsep{0pt}
\begin{center}
{\tiny mean pooling}
\end{center}

\end{minipage}};
% Text Node
\draw (152.32,108.97) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{33.35pt}\setlength\topsep{0pt}
\begin{center}
{\tiny mean pooling}
\end{center}

\end{minipage}};
% Text Node
\draw (194.86,39.05) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{10.89pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle E_{a}$
\end{center}

\end{minipage}};
% Text Node
\draw (194.86,81.41) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{11.21pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle E_{p}$
\end{center}

\end{minipage}};
% Text Node
\draw (194.73,119.67) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{11.52pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle E_{n}$
\end{center}

\end{minipage}};
% Text Node
\draw (227.55,107.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{42.42pt}\setlength\topsep{0pt}
\begin{center}
{\tiny increase distance}
\end{center}

\end{minipage}};
% Text Node
\draw (249.24,53.29) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{44.12pt}\setlength\topsep{0pt}
\begin{center}
{\tiny decrease distance}
\end{center}

\end{minipage}};
% Text Node
\draw (123.9,82.89) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{16.61pt}\setlength\topsep{0pt}
\begin{center}
{\tiny \textbf{BERT}}
\end{center}

\end{minipage}};
% Text Node
\draw (123.9,122.39) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{16.61pt}\setlength\topsep{0pt}
\begin{center}
{\tiny \textbf{BERT}}
\end{center}

\end{minipage}};


\end{tikzpicture}

==> src/pgfplots__Diagram__2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,487); %set diagram left start at 0, and has height of 487

%Right Arrow [id:dp7722752877802765] 
\draw   (392.02,-442.6) -- (392.13,-433.05) -- (395.46,-433.08) -- (388.87,-426.65) -- (382.14,-432.96) -- (385.47,-432.99) -- (385.36,-442.54) -- cycle ;
%Right Arrow [id:dp14060507328613792] 
\draw   (391.99,-403.76) -- (392.1,-394.21) -- (395.43,-394.24) -- (388.84,-387.82) -- (382.11,-394.13) -- (385.44,-394.16) -- (385.33,-403.71) -- cycle ;
%Image [id:dp9618221598010304] 
\draw (535.99,-405.65) node  {\includegraphics[width=103.32pt,height=84.14pt]{figures/rel-pred.png}};
%Shape: Ellipse [id:dp8909313910757333] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (583.7,-418.24) .. controls (583.7,-416.86) and (585.11,-415.74) .. (586.86,-415.74) .. controls (588.61,-415.74) and (590.02,-416.86) .. (590.02,-418.24) .. controls (590.02,-419.61) and (588.61,-420.73) .. (586.86,-420.73) .. controls (585.11,-420.73) and (583.7,-419.61) .. (583.7,-418.24) -- cycle ;
%Curve Lines [id:da0812705787316288] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (406.64,-342.72) .. controls (510.2,-300.13) and (581.78,-367.04) .. (586.52,-402.01) ;
\draw [shift={(586.69,-403.58)}, rotate = 94.53] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Right Arrow [id:dp982417144908057] 
\draw   (57.02,41.4) -- (57.13,50.95) -- (60.46,50.92) -- (53.87,57.35) -- (47.14,51.04) -- (50.47,51.01) -- (50.36,41.46) -- cycle ;
%Right Arrow [id:dp6478214650372898] 
\draw   (57.99,79.24) -- (58.1,88.79) -- (61.43,88.76) -- (54.84,95.18) -- (48.11,88.87) -- (51.44,88.84) -- (51.33,79.29) -- cycle ;
%Image [id:dp8496523532866038] 
\draw (201.99,77.35) node  {\includegraphics[width=103.32pt,height=84.14pt]{figures/rel-pred.png}};
%Shape: Ellipse [id:dp9281219922925783] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (249.7,64.76) .. controls (249.7,66.14) and (251.11,67.26) .. (252.86,67.26) .. controls (254.61,67.26) and (256.02,66.14) .. (256.02,64.76) .. controls (256.02,63.39) and (254.61,62.27) .. (252.86,62.27) .. controls (251.11,62.27) and (249.7,63.39) .. (249.7,64.76) -- cycle ;
%Straight Lines [id:da9089635748127332] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (60,150) -- (257,150) ;
%Straight Lines [id:da25090406964332956] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (257,150) -- (257,77) ;
\draw [shift={(257,74)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7831209160219743] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (60,150) -- (60,140) ;

% Text Node
\draw (360.36,-327.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{154.6pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize find distance of $\displaystyle E_{P}{}_{F}$ to refernce set using FAISS}
\end{center}

\end{minipage}};
% Text Node
\draw (348,-388.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{62.93pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Encode $\displaystyle E_{P}{}_{F}$ using }\\{\scriptsize fine-tuned BERT}
\end{center}

\end{minipage}};
% Text Node
\draw (354.32,-428) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{75.87pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Partial fact. e.g., \ $\displaystyle PF_{s}{}_{o} \ $}
\end{center}

\end{minipage}};
% Text Node
\draw (353.54,-466) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{55.49pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Test triple (s,p,o)}
\end{center}

\end{minipage}};
% Text Node
\draw (19.54,17) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{55.49pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Test triple (s,p,o)}
\end{center}

\end{minipage}};
% Text Node
\draw (19.32,58) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{47.88pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Partial fact $\displaystyle PF$}
\end{center}

\end{minipage}};
% Text Node
\draw (14,100.43) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{62.93pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Encode $\displaystyle E_{P}{}_{F}$ using }\\{\scriptsize fine-tuned BERT}
\end{center}

\end{minipage}};
% Text Node
\draw (30.36,163.43) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{154.6pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize find distance of $\displaystyle E_{P}{}_{F}$ to refernce set using FAISS}
\end{center}

\end{minipage}};


\end{tikzpicture}

